From anatomy to computation: axonal delay dispersion shifts neurons from event to sequence detection

Cortical neurons fire sparsely -- often fewer than one spike per sensory window -- so a neuron's spike count in that window carries little information, and its spike timing can carry more. That conduction delays convert firing order into synchrony is long established. What governs which class of temporal feature a neuron detects -- one volley of coincident input, or two in a particular order -- has not been examined. We propose a delay-signature framework in which the axonal conduction delays converging on a dendritic branch or a small neuron's soma constitute a physical key: only input sequences whose spike-time differences the delays compensate arrive synchronously, and coincidence detection, a threshold on input summed within an inhibition-compressed window, converts that synchrony into an all-or-none output. First, in simulations of an integrator-neuron model, a single physical scalar -- the dispersion of the delay set -- moves a population from event to order-selective sequence detection. The transition is emergent under random delays and connectivity, and an exact calculation reproduces it: at narrow dispersion, sequence detectors do not exist, and the dispersion at which they overtake event detectors tracks the inter-event interval. This maps a computational distinction onto the anatomical one between myelinated and unmyelinated projections, making myelination a switch on what a neuron computes. Second, the same dispersion sets the code's limits: it bounds the longest codable interval and fixes an absolute timing tolerance of order a millisecond, the same at every dispersion. Third, that millisecond window and the conduction velocity of afferents inside cortex together set column diameter, and column anatomy predicts the window measured in mouse barrel cortex. One anatomically measurable parameter thus shapes what a neuron detects and sets the limits of what it can represent.

==> preamble-preprint.tex <==

\journal{}
\makeatletter
\def\ps@pprintTitle{%
  \let\@oddhead\@empty \let\@evenhead\@empty
  \def\@oddfoot{\hfill\thepage\hfill}\let\@evenfoot\@oddfoot}
\makeatother

\usepackage{libertinus}
\usepackage[T1]{fontenc}
\usepackage{libertinust1math}

\hypersetup{colorlinks=true,
            linkcolor=[rgb]{0.05,0.20,0.50},
            citecolor=[rgb]{0.05,0.20,0.50},
            urlcolor=[rgb]{0.05,0.20,0.50}}

\usepackage[letterpaper,margin=1.35in,top=1in,bottom=1in]{geometry}
\linespread{1.06}
\usepackage{microtype}

\setlength{\abovecaptionskip}{6pt}
\setlength{\belowcaptionskip}{0pt}

\makeatletter
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \begingroup\footnotesize\linespread{1.0}\selectfont
  \sbox\@tempboxa{#1: #2}%
  \ifdim \wd\@tempboxa >\hsize
    #1: #2\par
  \else
    \global\@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \endgroup
  \vskip\belowcaptionskip}
\makeatother


